The Borel character

The main purpose of this article is to define a quadratic analog of the Chern character, the so-called Borel character, which identifies rational higher Grothendieck-Witt groups with a sum of rational MW-motivic cohomologies and rational motivic cohomologies. We also discuss the notion of ternary laws due to Walter, a quadratic analog of formal group laws, and compute what we call the additive ternary laws, associated with MW-motivic cohomology. Finally, we provide an application of the Borel character by showing that the Milnor-Witt K-theory of a field F embeds into suitable higher Grothendieck-Witt groups of F modulo explicit torsion.

==> hermitian.tex <==
%!TEX root = borel.tex

\subsection{Basics on hermitian K-theory and higher Witt groups}

\begin{df}\label{df:KQ}
Let $S$ be a scheme as in our conventions.
We will denote by $\KQ_S$ the motivic ring spectrum representing hermitian K-theory
 over $S$, denoted by $\mathbf{BO}$ in \cite{PW1}.
\end{df}
We need the following properties:
\begin{itemize}
\item[(GW1)] 
(\cite[Th. 1.2]{PW1}) 
Given any map $f:T \rightarrow S$, there is a canonical identification $f^*\KQ_S=\KQ_T$. In other words, $\KQ$
 is an absolute ring spectrum.
 This follows from the geometric model of hermitian K-theory using quaternionic
 Grassmanians.
\item[(GW2)]
(\cite[Cor.~7.3]{PW1})
For any regular scheme $S$ and any closed immersion $i : Z \to S$, there are isomorphisms:
\begin{equation}\label{eq:schlicht}
\KQ^{n,i}(S/S-Z)=\GW_{2i-n}^{[i]}(S \text{ on } Z)
\end{equation}
for all pairs $(n,i)\in\ZZ\times\ZZ$.
Here the right-hand side is Schlichting's higher Grothendieck--Witt groups:
 that is, the $(2i-n)$-th homotopy group of the spectrum
 $\mathbb GW^{[i]}(\mathcal A_S \text{ on } Z,\mathcal O_S)$ of \cite[Def. 8 of Section 10]{Schlicht1}.
 In the following, we will simply denote this spectrum by $\mathbb GW^{[i]}(S \text{ on } Z)$.
\end{itemize}

\begin{rem}
Under the twisting notation introduced for example in \cite{DJK},
 one can rewrite \eqref{eq:schlicht} as: $\KQ^{n}(S/S-Z, \dtw{i})=\GW_{n}^{[i]}(S~\text{on}~Z)$.
\end{rem}

The following result is well-known (see e.g. \cite{GepSna}):
\begin{prop}
Let $\E$ be a motivic ring spectrum over $S$.
 Consider a pair of integers $(n,i) \in \ZZ^2$.
 Then the following conditions are equivalent:
\begin{enumerate}
\item There exists an element $\rho \in \E_{n,i}(S)$, invertible for the cup-product
 on $\E_{**}$.
\item There exists an isomorphism: $\tilde \rho:\E(i)[n] \rightarrow \E$.
\end{enumerate}
\end{prop}

\begin{df}
A pair $(\E,\rho)$ satisfying the equivalent conditions of the above proposition will be called an \emph{$(n,i)$-periodic ring spectrum} over $S$.

An \emph{absolute} $(n,i)$-periodic ring spectrum is an $(n,i)$-periodic ring spectrum over $\Spec(\ZZp)$.\footnote{The restriction to $\Spec{\ZZp}$ comes
 from the global conventions of our paper. Needless to say the definition makes
 sense over $\Spec{\ZZ}$.}
\end{df}

\begin{prop}
There exists a family of elements $\rho_S \in \KQ^{8,4}(S)$ indexed by schemes,
 stable under pullback, such that $(\KQ_S,\rho_S)$ is $(8,4)$-periodic.
\end{prop}
This follows from the construction of the spectrum $\KQ_S$.
 The element $\rho_S$ can be defined using \cite[Prop. 7]{Schlicht1},
 which implies that there exists a canonical isomorphism of spectra:
$$
\mathbb GW^{[0]}(S) \simeq \mathbb GW^{[4]}(S).
$$
Therefore using (GW1),
 one gets an isomorphism: $\psi_S:\KQ^{0,0}(S) \xrightarrow{\sim} \KQ^{8,4}(S)$
 and we can put $\rho_S=\psi_S(1)$.

Following \cite{Anan1}, we introduce the following $\eta$-periodic spectra.
\begin{df}[Ananyevskiy]\label{df:KW}
Let $\eta:\un_S \rightarrow \un_S(-1)[-1]$ be the (desuspended) Hopf map.
 We define the $\eta$-periodized sphere spectrum $\un_S[\eta^{-1}]$ as:
$$
\un_S[\eta^{-1}]=\hocolim\big( \un_S \xrightarrow{\eta} \un_S(-1)[-1]
  \xrightarrow{\eta(-1)[-1]} \un_S(-2)[-2]  \xrightarrow{\eta(-2)[-2]} \hdots \big).
$$
Given any spectrum $\E$, we set $\E\wedge \un_S[\eta^{-1}]=\E[\eta^{-1}]$. In the special case of hermitian $K$-theory, we set $\KW_S=\KQ_S[\eta^{-1}]$. This defines an absolute ring spectrum.
\end{df}
In other words, $(\KW_S,\eta)$ is $(1,1)$-periodic.
 It is in fact the $(1,1)$-periodization of $\KQ_S$. Note also that the element
 $\rho_S \in \KQ^{8,4}(S)$ induces an element still denoted by $\rho_S \in \KW^{8,4}(S)$,
 and the above definition shows that $(\KW_S,\rho_S)$ is $(8,4)$-periodic.

Recall the following result of Ananyevskiy:

\begin{thm}[Ananyevskiy]
For any regular scheme $S$, there exists an isomorphism:
$$
\KW^{n,i}(S) \simeq W^{[i-n]}(S)
$$
where the right-hand side is Balmer's higher Witt groups.
\end{thm}

This is stated in \cite[Theorem~6.5]{Anan1} in the special case of smooth varieties, but the same proof applies here.
This isomorphism is contravariantly functorial in $S$, and induces an isomorphism of bigraded rings.

\begin{rem}
Over non-regular schemes, $\KQ$ and $\KW$ represent the $\AA^1$-invariant versions of higher Grothendieck--Witt and higher Witt groups, respectively.
\end{rem}

\subsection{Rational Borel isomorphism}

\begin{num}
As $\KW$ is $\eta$-periodic, the unit map $\un_S \rightarrow \KW_S$
 uniquely factors through a map
\begin{equation}
\label{eq:unit_KW}
\un_S[\eta^{-1}]\rightarrow \KW_S.
\end{equation}
The uniqueness of the factorization ensures that the latter map
 is a morphism of ring spectra.
\end{num}

\begin{num}\label{num:Morel_decomposition}
We fix an arbitrary base scheme $S$.
The symmetry involution permuting the factors  $\GG \wedge \GG$ induces an
 involution $\epsilon:\un_S \rightarrow \un_S$. We have two complementary projectors
 on $\un_S[1/2]$:
$$
e_+=\frac{1-\epsilon} 2, \phantom{i} e_-=\frac{1+\epsilon} 2,
$$
yielding Morel's decomposition: $\un_S[1/2]=\un_{S+} \oplus \un_{S-}$.
 More generally, given any spectrum $\E$ over $S$, we get a canonical decomposition:
$$
\E[1/2]=\E_+ \oplus \E_-
$$
such that $\epsilon$ acts by $+1$ (resp. $-1$) on $E_+$ (resp. $\E_-$).

Recall from Morel's computation that one has $\eta=\epsilon\eta$.
 In particular, we get:
$$
\un_S[1/2,\eta^{-1}]=\un_{S-}.
$$
In view of Definition \ref{df:KW}, we then deduce:
$$
\KQ_- \simeq \KW[1/2]=\KW_-.
$$

Recall that $(\KW_S,\rho_s)$ is $(8,4)$-periodic.
 One deduces a canonical map:
$$
\bigoplus_{m \in \ZZ} \un_S(4m)[8m] \xrightarrow{\sum_m \rho_S^m} \KW_S.
$$
Taking the rational parts and projecting this map to the minus part,
 we finally obtain a canonical map, uniquely determined by $\rho_S$:
$$
\psi_S:\bigoplus_{m \in \ZZ} \QQ_{S-}(4m)[8m] \xrightarrow{\sum_m \rho_S^m} \KW_{S,\QQ}.
$$
Note that by construction, the maps $\psi_S$ are compatible with pullbacks in $S$.
 The following result follows from \cite[Corollary~3.5]{ALP}.
\end{num}
\begin{thm}\label{thm:rational_witt}
For any scheme $S$, the map $\psi_S$ is an isomorphism.
\end{thm}
\begin{proof}
The formation of the map $\psi_S$ is compatible with base change.
 Recall from \cite[4.3.17]{CD3} that the family of functors $x^*$ for $x \in S$ a point of $X$
 is conservative. Thus we are reduced to the case where $S$ is the spectrum of a field
 (of characteristic different from $2$, since $S$ is a $\ZZp$-scheme by our conventions).
 Then the result follows from \cite[Corollary~3.5]{ALP}.
\end{proof}
%
%The following standard result, used in the proof above, does not require the assumptions of our global conventions.
%
%\begin{lm}
%\label{lm:point_conservative}
%Let $S$ be a noetherian scheme. For any point $x$ of $S$, denote by $i_x:\Spec{\kappa(x)} \rightarrow S$ the inclusion of the spectrum of the residue field. Then the family of functors $i_x^*:\SH(S)\to\SH(\kappa(x))$, for all points $x\in S$, is conservative.
%That is, a map $f$ in $\SH(S)$ is an isomorphism if and only if for every point $x\in S$, the map $i_x^*(f)$ is an isomorphism in $\SH(\kappa(x))$.
%\end{lm}
%
%\begin{proof}
%For any point $x$ of $S$, denote by $i'_x:\Spec{\mathcal{O}_{X,x}} \rightarrow S$ the canonical morphism. By \cite[Proposition 4.3.9]{CD3}, the family of functors $i'^*_x:\SH(S)\to\SH(\mathcal{O}_{X,x})$, for all points $x\in S$, is conservative. Therefore we may assume that $S$ has finite Krull dimension, and reduce to the case where $S$ is local when needed.
%
%We use the following notation: if $f:X\to Y$ is a morphism of schemes and $P\in\SH(Y)$, we denote by $P_{|X}$ the object $f^*P\in\SH(X)$. It suffices to prove that if $A\in\SH(S)$ is an object such that $A_{|x}\in\SH(\kappa(x))$ is $0$ for all points $x\in S$, then $A=0$. We argue by induction on the dimension of $S$: if $S$ has dimension $0$, then $S$ is a finite disjoint union of points and the claim is clear. Now suppose that the claim holds for schemes of dimension at most $n-1$. To prove the claim for schemes of dimension $n$, we are reduced to the case where $S$ is the spectrum of a local ring of dimension $n$. Denote by $i:x\to S$ the inclusion of the closed point and $j:U\to S$ the open complement. By the localization theorem we have a distinguished triangle in $\SH(S)$:
%$$
%j_!A_{|U}\to A\to i_*A_{|x}\to j_!A_{|U}[1].
%$$
%Since $U$ has dimension at most $n-1$, by the induction hypothesis, $A_{|U}=0$ and $A_{|x}=0$, which implies that $A=0$ in $\SH(S)$, and the result follows.
%\end{proof}

\begin{df}
We denote by
  \begin{equation*}
    \borel_{S,-} : \KW_{S,\QQ} \to \bigoplus_{m \in \ZZ} \QQ_{S-}(4m)[8m].
  \end{equation*}
the isomorphism of ring spectra inverse to $\psi_S$.
\end{df}

Before going further, we note the following remarkable corollary of the previous theorem.
\begin{cor}\label{cor:sp-orinted}
The absolute ring spectrum $\un_\QQ$ admits a canonical $\SL^c$-orientation over the category
 of $\ZZp$-schemes $S$.
 In particular, any rational ring spectrum over a $\ZZp$-scheme $S$
 admits a canonical $\SL^c$-orientation.
 In fact, $\un_\QQ$ is the universal $\SL^c$-orientable spectrum.
\end{cor}
Let us insist that in this corollary, we do not need the assumption that $S$ admits an ample
 family of line bundles.
\begin{proof}
Let $S$ be a $\ZZp$-scheme which admits an ample family of line bundles.

According to Example \ref{ex:orientations}, the ring spectrum $\KW_S$ is $\SL^c$-orientable over $S$.
 This implies that its rationalization $\KW_{S,\QQ}$ is $\SL^c$-orientable.
 Applying the previous theorem, $\un_{S,\QQ-}$ is a direct factor, as a ring spectrum,
 of $\KW_{S,\QQ}$. Therefore the $\SL^c$-orientation of $\KW_{S,\QQ}$ induces a canonical
 $\SL^c$-orientation on $\un_{S,\QQ-}$.
 In particular, we get such an $\SL^c$-orientation over $\Spec\left(\ZZp\right)$. By pullback,
 this is sufficient to get an $\SL^c$-orientation over the absolute ring spectrum $\un_{\QQ-}$
 over $\ZZp$-schemes.

Now, $\un_\QQ=\un_{\QQ+} \oplus \un_{\QQ-}$, as ring spectra. The plus part $\un_{\QQ+}$,
 being isomorphic to Beilinson motivic cohomology ring spectrum, is canonically orientable
 thus canonically $\SL^c$-orientable (Remark \ref{rem:link_orientations}).
 This gives the canonical orientation on $\un_\QQ$.

As every rational ring spectrum over $S$ is a ring extension of $\un_{S,\QQ}$, it acquire 
 a canonical $\SL^c$-orientation, and this concludes.
\end{proof}

\begin{rem}
It follows that rationally, the Thom space of a vector bundle $E/X$ depends only on the determinant of $E$.
 Similarly, any cohomology (resp. Borel-Moore homology) theory represented by a rational spectrum admits Gysin maps
 with respect to smoothable lci morphisms $f$
 up to a twist by the determinant of $f$, in the style of Chow-Witt groups (\cite{FaselCW}).
 Finally, the cohomology represented by the rational sphere spectrum in degree $(2r,r)$ of any regular $\ZZp$-scheme $S$
 is the rational Chow-Witt groups defined in \cite{FaselSrinivas}.

All these consequences will be drawn in details in \cite{DFJK3} and \cite{DFJK2}.
\end{rem}

%Using \cite{DJK} and the Sp-orientability from the previous corollary,
% one deduces the following result.
%\begin{cor}\label{cor:fdl}
%Let $\E$ be an arbitrary rational ring spectrum $\E$ over $S$.
% For a pair of integers $(n,i) \in \ZZ^2$, a $S$-scheme $X$ with structural map $p$
% (resp. $p$ separated of finite type),
% and a line bundle $L$ over $X$, one puts:
%\begin{align*}
%\E^{n,r}(X,L)&=\Hom_{\SH(S)}(\un_X,p^*\E(r)[n] \otimes \Th_S(L)), \\
%\text{resp. } \E_{n,r}(X/S,L)&=\Hom_{\SH(S)}(\un_X(r)[n] \otimes \Th_S(L),p^!\E).
%\end{align*}
%Then for any smoothable lci morphism
%  $f:X \rightarrow S$ of relative virtual dimension $r$,
% there exists a fundamental class $\eta_f \in \E_{n,r}(X/S,\det{L_f})$.
% Altogether, these fundamental classes satisfy
% compatibility with composition and the excess intersection formula.
%\end{cor}

\begin{num}
Let again $S$ be an arbitrary scheme.
 Recall from \cite[Th. 3.4]{RonOst} that one has a canonical distinguished triangle:
$$
\KQ_S(1)[1] \xrightarrow{\eta} \KQ_S \xrightarrow f \KGL_S \rightarrow \KQ_S(1)[2]
$$
where $\KGL$ is the spectrum representing the homotopy invariant $K$-theory over $S$
 and $f$ the \emph{forgetful map}.

As $\eta_+=0$ and $\KGL_{S-}=0$, we immediately deduce the following result.
\end{num}
\begin{prop}
One has a split exact sequence in $\SH(S)[1/2]$, and more precisely in $\SH(S)_+$,
 the essential image of the projector $e_+$ of Paragraph \ref{num:Morel_decomposition}:
$$
0 \rightarrow \KQ_{S+}
 \xrightarrow f \KGL_S[1/2] \rightarrow \KQ_{S+}(1)[2] \rightarrow 0.
$$
In other words, $\KGL_S[1/2] \simeq \KQ_{S+} \oplus \KQ_{S+}(1)[2]$.
\end{prop}
There is moreover a canonical splitting of the above map. Indeed, consider the ``twisted'' forgetful map
\[
f(1)[2]: \KQ_{S,+}(1)[2]\to  \KGL_S(1)[2]\simeq  \KGL_S
\]
Then, the composite 
\[
\KQ_{S,+}(1)[2]\xrightarrow{f(1)[2]}  \KGL_S\xrightarrow{H}  \KQ_{S+}(1)[2]
\]
is just multiplication by $2$ and $\frac 12f(1)[2]$ is a section of $H$.

Recall from \cite{Riou, CD3} that the classical Chern character corresponds to an
 isomorphism of the following form in $\SH(S)$:
$$
\ch:\KGL_{S,\QQ} \rightarrow \bigoplus_{m \in \ZZ} \QQ_{S+}(m)[2m]
$$
where $\QQ_{S+}$ is identified with the rational motivic Eilenberg-MacLane spectrum
 (equivalently, the universal orientable ring spectrum).
\begin{prop}
The composition
$$
\KQ_{S,\QQ+} \xrightarrow f \KGL_{\QQ,S}
 \xrightarrow{\ch} \bigoplus_{m \in \ZZ} \QQ_{S+}(m)[2m]
$$
induces an isomorphism
$$
\KQ_{S,\QQ+} \xrightarrow{\borel_{S,+}} \bigoplus_{m \in \ZZ} \QQ_{S+}(2m)[4m].
$$ 
\end{prop}
\begin{proof}
According to \cite{Schlicht1},
 there is an isomorphism $\mathbb GW^{[0]} \simeq \mathbb GW^{[2]}_\epsilon$
 where $\epsilon$ consists in taking the opposite duality.
 In particular, we get an isomorphism of functors
 $\mathbb GW^{[0]} \simeq \mathbb GW^{[4]}$ and, using the isomorphism \eqref{eq:schlicht},
 one deduces there is an element $\sigma_S \in \KQ_+^{4,2}(S)$
 such that $(\KQ_+,\sigma_S)$ is $(4,2)$-periodic.
 By construction, one has $\sigma_S^2=\rho_S$ and one can check that $f(\sigma_S)=\beta^2$,
 where $\beta$ is the Bott element in K-theory (expressing its (2,1)-periodicity).
 This finishes the proof.
\end{proof}

\begin{num}
In particular, one gets a canonical isomorphism:
\begin{equation}\label{eq:pontryagin}
\begin{split}
\KQ_{S,\QQ} 
\simeq 
&\KQ_{S,\QQ+} \oplus \KQ_{S,\QQ-}\\
 \xrightarrow{\borel_{S,+} \oplus \borel_{S,-}} 
&\bigoplus_{m \in \ZZ} \QQ_{S+}(2m)[4m]
 \oplus \bigoplus_{m \in \ZZ} \QQ_{S-}(4m)[8m],
\end{split}
\end{equation}
which, from the above constructions, is in fact an isomorphism of ring spectra.
\end{num}
\fz{It seems to me that we can define the inverse of~\eqref{eq:pontryagin} with $\ZZ[1/2]$-coefficients: the canonical map
\begin{align}
\ZZ[1/2]_{S+}\to \KQ_{S,\ZZ[1/2]+}
\end{align}
extends to $\bigoplus_{m \in \ZZ} \ZZ[1/2]_{S+}(2m)[4m]$ by $(4,2)$-periodicity. Gluing with the negative part we get
\begin{align}
\bigoplus_{m \in \ZZ} \ZZ[1/2]_{S+}(2m)[4m]
\oplus
\bigoplus_{m \in \ZZ} \ZZ[1/2]_{S-}(4m)[8m]
\to
\KQ_{S, \ZZ[1/2]}
\end{align}
which is rationally an isomorphism.
}
\begin{df}\label{df:Borel}
We call the above isomorphism the \emph{Borel character} and denote it by 
\[
\borel_S:\KQ_{S,\QQ}\to \bigoplus_{m \in \ZZ} \QQ_{S+}(2m)[4m]
 \oplus \bigoplus_{m \in \ZZ} \QQ_{S-}(4m)[8m].
\]
\fz{Note that $\QQ_{S-}=\nu_*\QQ_{S_\QQ-}$ by the result of the other paper.}
\end{df}


